Don't Be Greedy: Leveraging Community Structure to Find High Quality Seed Sets for Influence Maximization

We consider the problem of maximizing the spread of influence in a social network by choosing a fixed number of initial seeds --- a central problem in the study of network cascades. The majority of existing work on this problem, formally referred to as the influence maximization problem, is designed for submodular cascades. Despite the empirical evidence that many cascades are non-submodular, little work has been done focusing on non-submodular influence maximization. We propose a new heuristic for solving the influence maximization problem and show via simulations on real-world and synthetic networks that our algorithm outputs more influential seed sets than the state-of-the-art greedy algorithm in many natural cases, with average improvements of 7% for submodular cascades, and 55% for non-submodular cascades. Our heuristic uses a dynamic programming approach on a hierarchical decomposition of the social network to leverage the relation between the spread of cascades and the community structure of social networks. We verify the importance of network structure by showing the quality of the hierarchical decomposition impacts the quality of seed set output by our algorithm. We also present "worst-case" theoretical results proving that in certain settings our algorithm outputs seed sets that are a factor of $\Theta(\sqrt{n})$ more influential than those of the greedy algorithm, where $n$ is the number of nodes in the network. Finally, we generalize our algorithm to a message passing version that can be used to find seed sets that have at least as much influence as the dynamic programming algorithms.

==> message-passing.tex <==
In this section we describe a Message Passing Algorithm (\algo{MPA}), formally presented in Algorithm \ref{algo:mpa}, which is a generalization of  \algo{DPIM}.  This algorithm provides a new perspective on  \algo{DPIM}, and can be made to perform strictly better at the cost of additional run time.

\paragraph{Notation:} First, we must present notation that we will use to formally describe
\algo{MPA}.  Define $L(v_T), R(v_T),$ and $U(v_T)$ to be the left child of
$v_T$, right child of $v_T$, and the parent of $v_T$, respectively. We use $D$
as a placeholder for an element in $\{L, R\}$ (down directions) and $\mathfrak{D}$ as a
placeholder for an element in $\{L, R, U\}$ (all directions).  (Note that
we use $D(v_T)$ and $\mathfrak{D}(v_T)$ as a generalization of the above.)
Lastly, let $T_\mathfrak{D}(v_T) = T(\mathfrak{D}(v_T))$ and $\mathbb{D} =
\{(L,R), (L,U), (R,U) \}$.

Furthermore, we define the return direction for a node, $v_T \in
V_T$, by $\mathfrak{R}^{(v_T)}_\mathfrak{D} \in \{L, R, U\}$ such that
$\mathfrak{R}^{(v_T)}_\mathfrak{D}(\mathfrak{D}(v_T)) = v_T$. Naturally, define $\neg
\mathfrak{R}^{(v_T)}_\mathfrak{D} \in \mathbb{D}$ such that neither of the
coordinates of $\neg \mathfrak{R}^{(v_T)}_\mathfrak{D}$ are
$\mathfrak{R}^{(v_T)}_\mathfrak{D}$.

\paragraph{Data Structure:} \algo{MPA} will sequentially, locally update a data-structure, which we describe
now. Let $A: V_T \times \mathbb{D} \times [k] \rightarrow [k] \times [k]$
where both output coordinates of $A(v_T, (\mathfrak{D}_1, \mathfrak{D}_2), \ell)$ are non-negative integers that sum to at most $\ell$.
Intuitively, $A(v_T, (\mathfrak{D}_1, \mathfrak{D}_2), \ell)$ answers:  how
should  $\ell$ seeds should be split between $T_{\mathfrak{D}_1}(v_T)$ and
$T_{\mathfrak{D}_2}(v_T)$? The answer is that we should put  $A(v_T,
(\mathfrak{D}_1, \mathfrak{D}_2), \ell)_i$ seeds in $T_{\mathfrak{D}_i}(v_T)$ for
each $i \in \{1, 2\}$. Note that for the root vertex $r \in V_T$, which has no parent, we insist that  $A(r,
(D,U), \ell)_2 = 0$.

%For notational reasons, we now define:
%$\neg_1 L = R$, $\neg_2 L = P$, $\neg_1 R = L$, $\neg_2 R = P$, $\neg_1 P = L$, $\neg_2 P = R$.

\paragraph{Obtaining a Seed Set:}Once we have such a data-structure $A$, we define a function that answers the more natural question:
Let $B: V_T \times \mathbb{D} \times [k] \rightarrow 2^V$ where
$B(v_T,  (\mathfrak{D}_1,\mathfrak{D}_2), \ell)$ is a subset of $
T_{\mathfrak{D}_1}(v_T) \cup T_{\mathfrak{D}_2}(v_T)$ of at most $\ell$
vertices.  Intuitively, the question that $B$ answers is: where should the
allocation of $\ell$ vertices in $T_{\mathfrak{D}_1}(v_T) \cup T_{\mathfrak{D}_2}(v_T)$ be placed?

Given a filled instance of $A$, $B(v_T, \mathfrak{D}_1, \mathfrak{D}_2, \ell)$  recursively follows the advice of $A$ in
placing seeds in $T_{\mathfrak{D}_1}(v_T)$ and $T_{\mathfrak{D}_2}(v_T)$. We
divide the definition of $B(v_T, (\mathfrak{D}_1, \mathfrak{D}_2), \ell)$ into two
cases:

\begin{enumerate}[I)]
\item $(\mathfrak{D}_1, \mathfrak{D}_2) = (L, R)$: If $v_T$ is a leaf node, then
$$B(v_T, (L,R), \ell) = \left\{ \begin{array}{cc} T(v_T) &  \ell \geq 1 \\
\emptyset & \ell = 0 \end{array}.\right.$$
Otherwise, 
\begin{align*}
B(v_T, (L,R), \ell) = & B(L(v_T), (L,R), A[v_T, (L,R), \ell]_1) \; \cup \\ &B(R(v_T),
(L,R), A[v_T, (L,R), \ell]_2).
\end{align*}
\item $(\mathfrak{D}_1, \mathfrak{D}_2) = (D, U)$: If $v_T = r$, the root of
$T$, then 
$$B(v_T, (D,U), \ell) = B(D(v_T), (L,R), \ell).$$
If $v_T$ is a leaf node, then
\begin{align*}
B(v_T, (D,U), l) = & B(v_T, (L, R), A(v_T, (D, U), l)_1) \; \cup \\
& B(U(v_T), \neg \mathfrak{R}^{(v_T)}_D, A(v_T, (D, U), l)_2).
\end{align*}
Otherwise, 
\begin{align*}
B(v_T, (D,U), l) = & B(D(v_T), (L, R), A(v_T, (D, U), l)_1) \; \cup \\
& B(U(v_T), \neg \mathfrak{R}^{(v_T)}_D, A(v_T, (D, U), l)_2).
\end{align*}

\end{enumerate}


%Second, if $v_T = r_T$, then:
%$$B(v_T, DU, \ell) = B(D(v_T), LR, \ell)$$
%
%\gs{We have better notation for this later. Also, this is incorrect!}
%
%Given $v_T \in T$, $D \in \{L, R, U\}$ define $R^{v_T, D} \in \{L, R, U\}$  $v_T = R^{v_T, D}(D(v_T))$ so if you leave $v_T$ in direction $D$ you return in direction $R^{v_T, D}$.  Let $ \neg R^{v_T, D} \in \{LU, RU, LR\}$ denote the two directions that do not return to $v_T$.



%otherwise define:
%\begin{align*}
%B(v_T, DU, \ell) = & B(D(v_T), LR, A[v_T, DU, \ell]_1) \cup  \\
%                    &B(U(v_T), \neg R^{v_T, U}, A[v_T, DU, \ell]_2).
%\end{align*}
%
%%$$B(v_T, DU, \ell) = B(D(v_T), LR, A[v_T, DU, \ell]_1) \cup B(U(v_T), D'U, A[v_T, DU, \ell]_2).$$

\noindent Note that $B(r, (L,R), k)$ denotes where to place $k$ initial seeds over all of $V$.

\paragraph{Local Update Subroutine:} Now that we have defined $A$ and shown how it defines initial seeds sets,  we
will define a way to locally update $A$ to improve the allocation.  The idea is
just this, to update  $A(v_T, (\mathfrak{D}_1, \mathfrak{D}_2), \ell)$, try all possible outputs whose
coordinates sum to $\ell$ and return the best.  Let $\mathfrak{D}_3$ be the sole
element of ${\{ L, R, U\} \setminus\{\mathfrak{D}_1, \mathfrak{D}_2}\}$.  We
will first allocate $k - \ell$ vertices to $T_{\mathfrak{D}_3} (v_T)$ according to $A$.
Next, try the different divisions between $T_{\mathfrak{D}_1}(v_T)$ and
$T_{\mathfrak{D}_2}(v_T)$ for the remaining $\ell$ vertices. This procedure is
formally defined in Algorithm \ref{algo:update}.
%
% $R_1^{v_T, D} \neq D_2^{v_T, D} \in  \{L, R, U\}$ such that  $v_T \not\in T_{R_1^{v_T, D}}(D_3(v_T)) \cup T_{R_2^{v_T, D}}(D_3(v_T))$.  This is to say that $R_1^{v_T, D}$, $ D_2^{v_T, D}
%
% $R_1^{v_T, D}$  $D_2^{v_T, D}$
%Let $D_1' \neq D_2'$ be such that $v_T \not\in T_{D_1'}(D_3(v_T)) \cup T_{D_2'}(D_3(v_T))$


\begin{algorithm}[h!]\label{alg}
\SetAlgoNoLine
\KwIn{$I = (G = (V, E), T = (V_T, E_T), \sigma(\cdot), k), A, v_T,
(\mathfrak{D}_1, \mathfrak{D}_2) \in \mathbb{D}$} % input
\KwOut{An updated instance of $A$} % output
Let $\mathfrak{D}_3$ be the sole element of $\{ L, R, U\} \setminus\{\mathfrak{D}_1,
\mathfrak{D}_2\}$.\\
%Let $D_1' \neq D_2'$ be such that $\{  \}
%
%$v_T \not\in T_{D_1'}(D_3(v_T)) \cup T_{D_2'}(D_3(v_T))$
%If $v_T \neq r_T$ then let $D'$ denote the child that $v_T$ is of its parent: so that $v_T = D'(U(v_T))$

%$\algo{update}(I, A, v_T, D_1, D_2) = $\\
 \For{each $i = 0, 1, \ldots, k$}{
        $j = \argmax\limits_{ j \in \{0, 1,\ldots, i\}}
        \sigma\left(
        B\left(\mathfrak{D}_1(v_T),\neg R^{(v_T)}_{\mathfrak{D}_1}, j\right) \cup
        B\left(\mathfrak{D}_2(v_T),\neg R^{(v_T)}_{\mathfrak{D}_2},
        i-j\right) \cup B\left(\mathfrak{D}_3(v_T), \neg R^{(v_T)}_{\mathfrak{D}_3},
        k-i\right) \right)$\\
        $A(v_T, (\mathfrak{D}_1, \mathfrak{D}_2), i) := (j, i -j)$ \\
       }
  \Return{A}
\caption{\algo{update}: Local Update Subroutine}
\label{algo:update}
\end{algorithm}
\gs{add caption}

\begin{algorithm}[h!]\label{alg}
\SetAlgoNoLine
\KwIn{$I = (G = (V, E), T = (V_T, E_T), \sigma(\cdot), k)$} % input
\KwOut{$S$, a set of $k$ nodes of $V$}%$B(r_T, LR, k)$} % output
Let $A(\cdot) = (0, 0)$ \\
\For{each height $i = 1, 2, \ldots h$} {
  \For{each node $v_T \in V_T$ with height $i$} {
      $\algo{update}(I, A, v_T, (L, R));$\\
  }
}
Let $S, S' := B(r_T, (L, R), k)$;\\
\Do{$\sigma(S') > \sigma(S)$}{
%\While{$\sigma(B(r_T, LR, k))$ is increasing } {
  S := S';\\
  \For{each height $i = h-1, \ldots, 1$} {
    \For{each node $v_T \in V_T$ with height $i$} {
      $\algo{update}(I, A, v_T, (L, U))$;\\
      $\algo{update}(I, A, v_T, (R, U))$;
    }
  }
  \For{each height $i = 1, 2, \ldots h$} {
    \For{each node $v_T \in V_T$ with height $i$} {
      $\algo{update}(I, A, v_T, (L, R));$\\
    }
  }
  $S' = B(r_T, (L, R), k)$;
}
\Return{$B(r_T, (L, R), k)$}
\caption{\algo{MPA}: Message Passing Algorithm}
\label{algo:mpa}
\end{algorithm}

\paragraph{Generalizing \algo{DPIM}:} Given that we have our local update, we
need only define: (a) an initial configuration of $A$, (b) a sequence of
updates, and (c) a terminating condition (if the sequence is infinite). 
For example, our  \algo{DPIM} is a special case where every entry in $A$ is $(0, 0)$
initially, and then we update $A(v_T, (L,R), \cdot)$ by going up the tree.


In Algorithm~\ref{algo:mpa}, we give another possible schedule where we go up
and down the tree until no additional improvements are found. Given a graph, decomposition, 
influence function, $k$, and current allocation $A$, we run \algo{DPIM} to
initialize $A$.  Then, we evaluate each node on each level of $T$ down and up
the tree, finishing at the root node, checking whether there has been any
improvements in the influence of the seed sets, and repeating until there are no
more improvements. Note that this algorithm must terminate, since it would be
implemented using a finite precision approximation of $\sigma(\cdot)$.



%Note that this algorithm first runs \algo{DPIM}.  Then it goes up and down the tree until no more improvements are calculated.
%
%%%
%%%
%%%First, if $v_T = r_T$, then:
%%%$$B(v_T, LR, \ell) = B(L(v_T), LR, A[v_T, LR, \ell]_1) \cup B(R(v_T), LR, A[v_T, LR, \ell]_2)$$.
%%%$$B(v_T, DU, \ell) = B(D(v_T), LR, A[v_T, DU, \ell]_1) \cup B(U(v_T), D'U, A[v_T, DU, \ell]_2)$$.
%%%
%%%First, if $v_T \not\eq r_T$ let $D' \{R, L\}$ denote the child that $v_T$ is of its parent: so that $v_T = D'(U(v_T))$.  Then:
%%%$$B(v_T, LR, \ell) = B(L(v_T), LR, A[v_T, LR, \ell]_1) \cup B(R(v_T), LR, A[v_T, LR, \ell]_2)$$.
%%%$$B(v_T, DU, \ell) = B(D(v_T), LR, A[v_T, DU, \ell]_1) \cup B(U(v_T), D'U, A[v_T, DU, \ell]_2)$$.
%%
%%
%%
%%
%%
%%
%%
%%
%%
%%
%%%
%%%Intuitively, $A[v_T, D, \ell]$ answers: if $k-\ell$ seeds are placed in $T_D(v_T)$, then how should the remaining $ell$ seeds should be split between $T_{\neg_1 D}(v_T)$ and $T_{\neg_2 D}(v_T)$?  The answer is that we should put  $A[v_T, D, \ell]$ seeds in $T_{\neg_1 D}(v_T)$ and the remaining $\ell - A[v_T, D, \ell]$ seeds in $T_{\neg_2 D}(v_T)$.
%%%
%%%Once we have such a data-structure $A$, we can build a data-structure that answers the more natural question:
%%%Let $B: V_T \times \{L, R, P\} \times [k] \rightarrow 2^V$ where $B(v_T, D, \ell)$ is a subset of $V \setminus T_D(v_T)$ of at most $\ell$ vertices.  Intuitively the question that $B$ answers is: if I allocate $\ell$ vertices to $T_D(v_T)$, where should they be placed.
%%%
%%%Given an $A$, we construct $B$ as follows:
%%%
%%%$$B(v_T, D, \ell) = B(\neg_1 D(v_T), D, A[v_T, D, k -\ell]) \cup B(\neg_2 D(v_T), D,  \ell - A[v_T, D, k-\ell])$$.  Recall that $A$ tells us how to allocate  so here we see that if we allocate $\ell$ vertices to $T_D(v_T)$, then
%%
%%%Intuitively, $A[v_T, D, \ell]$ answers: if $k-\ell$ seeds are placed in $T_D(v_T)$, then how should the remaining seeds should be split between $T_{\neg_1 D}(v_T)$ and $T_{\neg_2 D}(v_T)$?  The answer is that we should put  $A[v_T, D, \ell]$ seeds in $T_{\neg_1 D}(v_T)$ and the remaining $k - \ell - A[v_T, D, \ell]$ seeds in $T_{\neg_2 D}(v_T)$.
%%
%%%Once we have such a data-structure $A$, we can build a data-structure that answers the more natural question:
%%%Let $B: V_T \times \{L, R, P\} \times [k] \rightarrow 2^V$ where $B(v_T, D, \ell)$ is a subset of $V \setminus T_D(v_T)$ of at most $\ell$ vertices.  Intuitively the question that $B$ answers is: if I allocate $\ell$ vertices to $V \setminus T_D(v_T)$, where should the \emph{remaining} $k - \ell$ vertices be placed.  Of course, this sounds a little backwards, but this is the correct way to define things.
%%
%%
%%%Given an $A$, we construct $B$ as follows:
%%%
%%%$$B(v_T, D, \ell) = B(\neg_1 D(v_T), D, A[v_T, D, \ell]) \cup B(\neg_2 D(v_T), D, k - \ell - A[v_T, D, \ell])$$  so here we see that if we allocate $\ell$ vertices to $T_D(v_T)$, then
%%
%%
%%  a current set of (at most) $\ell$ vertices in in $v_D(v_T)$ that the algorithm will infect.  Our update algorithm will update $A$ for one vertex and direction at a time.
%%
%%
%%Let $A: V_T \times \{L, R, P\} \times [k] \rightarrow 2^V$ where $A(v_T, D, \ell)$ is a subset of $T_D(v_T)$ of at most $\ell$ vertices.
%%Recall that $T_L(v_T)$, $T_R(v_T)$ are the left and right subtrees of $T(v_T)$ and $T_P(v)$ is the remaining vertices.
%%
%%Intuitively, $A$ records a current set of (at most) $\ell$ vertices in in $v_D(v_T)$ that the algorithm will infect.  Our update algorithm will update $A$ for one vertex and direction at a time.
%%
%%Given a graph, decomposition, influence function, $k$, and current allocation $A$, we update $A$ for
%%
%%\begin{algorithm}[h!]\label{alg}
%%\SetAlgoNoLine
%%\KwIn{$I = (G = (V, E), T = (V_T, E_T), \sigma(\cdot), k), A, v_T \in V_T, D \in \{L, R, P\}$} % input
%%\KwOut{A} % output
%%$UPDATE(I, A, v_T, D) = $\\
%%
%% \For{each $i = 0, 1, \ldots, k\}$}{
%%        $j = \argmax\limits_{ j \in \{0, 1,\ldots, i\}} \sigma(A[v_T, \neg_1 D, j] \cup
%%        A[v_T,\neg_2 D, i-j] \cup B[v_P, k - i])$\\
%%        $A_P[v_T, i] = A_P[v_L, j] \cup A_P[v_R, i-j]$
%%      }
%%
%%
%%For a node $v_T \in V_T$, let $v_R, v_L,$ and $v_P$ be the left child, right child and parent of $v_T$, resp.
%%Let $A_P[ \cdot , \cdot ] = V_T \times [k] \to 2^V$, such that $A_P[v_T,j]$ stores a
%%choice of $j$ seeds in $T(v_T)$.  \\
%%Let $A_L[ \cdot , \cdot ] = V_T \times [k] \to 2^V$, such that $A_L[v_T,j]$ stores a
%%choice of $j$ seeds in $V \setminus T(v_L)$.  \\
%%Let $A_R[ \cdot , \cdot ] = V_T \times [k] \to 2^V$, such that $A_R[v_T,j]$ stores a
%%choice of $j$ seeds in $V \setminus T(v_R)$.  \\
%%Let $r \in V_T$ be the root of $T$ and $h$ be its height.\\
%%Run \algo{DPIM} on the input parameters, except return $A$ instead of the seed
%%set. \\
%%$A_P := A$ \\
%%\While{$\sigma(A_P[r, k])$ is increasing } {
%%  \For{each height $i = h - 1, h - 2, \ldots, 1, 2, \ldots h - 1$} {
%%    \For{each node $v_T \in V_T$ with height $i$} {
%%      \eIf{$v_T$ is the left child of $v_P$}{
%%        $B := A_L$
%%      }{
%%        $B := A_R$
%%      }
%%      \For{each $i = 0, 1, \ldots, \min\{|T(v_T)|, k\}$}{
%%        $j = \argmax\limits_{ j \in \{0, 1,\ldots, i\}} \sigma(A_P[ v_L,j] \cup
%%        A_P[ v_R, i-j] \cup B[v_P, k - i])$\\
%%        $A_P[v_T, i] = A_P[v_L, j] \cup A_P[v_R, i-j]$
%%      }
%%      \For{each $i = 0, 1, \ldots, \min\{|T(v_T)|, k\}$}{
%%        $j = \argmax\limits_{ j \in \{0, 1,\ldots, i\}} \sigma(B[ v_P,j] \cup
%%        A_P[ v_R, i-j] \cup A_P[v_L, k - i])$\\
%%        $A_L[v_T, i] = B[v_P, j] \cup A_P[v_R, i-j]$
%%      }
%%      \For{each $i = 0, 1, \ldots, \min\{|T(v_T)|, k\}$}{
%%        $j = \argmax\limits_{ j \in \{0, 1,\ldots, i\}} \sigma(A_P[ v_L,j] \cup
%%        B[ v_P, i-j] \cup A_P[v_R, k - i])$\\
%%        $A_R[v_T, i] = A_P[v_L, j] \cup B[v_P, i-j]$
%%      }
%%    }
%%  }
%%}
%%\Return{$A_P[r, k]$}
%%\caption{\algo{MPA}: Message Passing Algorithm}
%%\label{algo:mpa}
%%\end{algorithm}
%
%
%
%\gs{add to prelims}
%For each vertex $v_T \in V_T$ in the hierarchical decomposition, we divide the
%network into three induced subnetworks: the left subtree $T_L(v_T)$, the right subtree $T_R(v_T)$, and parents tree $T_P(v_T) \equiv V \setminus T(v)$ corresponding to the three ``directions" one can travel from $v_T$.
%
%
%%For each vertex $v \in V_T$ in the hierarchical decomposition, we divide the
%%network into three induced subnetworks: $T_L(v) \equiv T(L(v))$, $T_R(v) \equiv T(R(v))$, and $T_P(v) \equiv T_R(v) V \setminus (T(v))$ corresponding to the three ``directions": left, right, and parent one can travel from $v_T$.
%
%For each vertex $v_T$ in the hierarchical decomposition, we divide the
%network into three induced subnetworks, related to the parent, left child, and
%right child of $v_T$, and compare the total influence of various seed sets
%across these subnetworks.  Let $v_L$ and $v_R$ be the left and right child of any
%node $v_T \in V_T$.  Divide the network into three induced subnetworks defined
%implicitly by $T(v_L)$, $T(v_R)$, and $V \setminus T(v_T)$, corresponding to the left
%sub-community of $T(v_T)$, the right sub-community of $T(v_T)$, and the rest of
%the network, respectively.
%
%
%
%Next, we compare how the different combinations of high-quality
%seed sets within each of these subnetworks work in tandem, choosing the union
%that maximizes the total influence.  We repeat this process for each node on
%each level going up and down the levels of the hierarchical decomposition until
%we no longer are improving the total influence of the best seed set (checking
%the total influence each time we reach the root node of the hierarchical
%decomposition).
%
%
%
%After considering the quality of seed sets that
%\algo{DPIM} finds in comparison to the greedy algorithm, it is natural to ask if
%we can develop an effective algorithm that is deliberately designed to find seed sets that create
%inter-community synergies. In light of the success of $\algo{DPIM}$, we present a
%Message Passing Algorithm (\algo{MPA}), formally presented in Algorithm \ref{algo:mpa}.
%
%At a high-level, \algo{MPA} works as follows.
%For each vertex $v_T$ in the hierarchical decomposition, we divide the
%network into three induced subnetworks, related to the parent, left child, and
%right child of $v_T$, and compare the total influence of various seed sets
%across these subnetworks.  Let $v_L$ and $v_R$ be the left and right child of any
%node $v_T \in V_T$.  Divide the network into three induced subnetworks defined
%implicitly by $T(v_L)$, $T(v_R)$, and $V \setminus T(v_T)$, corresponding to the left
%sub-community of $T(v_T)$, the right sub-community of $T(v_T)$, and the rest of
%the network, respectively. Next, we compare how the different combinations of high-quality
%seed sets within each of these subnetworks work in tandem, choosing the union
%that maximizes the total influence.  We repeat this process for each node on
%each level going up and down the levels of the hierarchical decomposition until
%we no longer are improving the total influence of the best seed set (checking
%the total influence each time we reach the root node of the hierarchical
%decomposition).
%
%In addition, MPA will always converge, since there is a fixed finite maximum
%amount of total influence possible and finite precision will be used to store the value
%of total influence.
%
%
%% Message-Passing Algorithm
%\begin{algorithm}[h!]\label{alg}
%\SetAlgoNoLine
%\KwIn{$G = (V, E), T = (V_T, E_T), \sigma(\cdot), k$} % input
%\KwOut{$S \subset V$ such that $|S| = k$ %and $S$ maximizes $\sigma(\cdot)$ over the subsets of nodes associated with the nodes of $\mathcal{D}$
%} % output
%For a node $v_T \in V_T$, let $v_R, v_L,$ and $v_P$ be the left child, right child and parent of $v_T$, resp.
%Let $A_P[ \cdot , \cdot ] = V_T \times [k] \to 2^V$, such that $A_P[v_T,j]$ stores a
%choice of $j$ seeds in $T(v_T)$.  \\
%Let $A_L[ \cdot , \cdot ] = V_T \times [k] \to 2^V$, such that $A_L[v_T,j]$ stores a
%choice of $j$ seeds in $V \setminus T(v_L)$.  \\
%Let $A_R[ \cdot , \cdot ] = V_T \times [k] \to 2^V$, such that $A_R[v_T,j]$ stores a
%choice of $j$ seeds in $V \setminus T(v_R)$.  \\
%Let $r \in V_T$ be the root of $T$ and $h$ be its height.\\
%Run \algo{DPIM} on the input parameters, except return $A$ instead of the seed
%set. \\
%$A_P := A$ \\
%\While{$\sigma(A_P[r, k])$ is increasing } {
%  \For{each height $i = h - 1, h - 2, \ldots, 1, 2, \ldots h - 1$} {
%    \For{each node $v_T \in V_T$ with height $i$} {
%      \eIf{$v_T$ is the left child of $v_P$}{
%        $B := A_L$
%      }{
%        $B := A_R$
%      }
%      \For{each $i = 0, 1, \ldots, \min\{|T(v_T)|, k\}$}{
%        $j = \argmax\limits_{ j \in \{0, 1,\ldots, i\}} \sigma(A_P[ v_L,j] \cup
%        A_P[ v_R, i-j] \cup B[v_P, k - i])$\\
%        $A_P[v_T, i] = A_P[v_L, j] \cup A_P[v_R, i-j]$
%      }
%      \For{each $i = 0, 1, \ldots, \min\{|T(v_T)|, k\}$}{
%        $j = \argmax\limits_{ j \in \{0, 1,\ldots, i\}} \sigma(B[ v_P,j] \cup
%        A_P[ v_R, i-j] \cup A_P[v_L, k - i])$\\
%        $A_L[v_T, i] = B[v_P, j] \cup A_P[v_R, i-j]$
%      }
%      \For{each $i = 0, 1, \ldots, \min\{|T(v_T)|, k\}$}{
%        $j = \argmax\limits_{ j \in \{0, 1,\ldots, i\}} \sigma(A_P[ v_L,j] \cup
%        B[ v_P, i-j] \cup A_P[v_R, k - i])$\\
%        $A_R[v_T, i] = A_P[v_L, j] \cup B[v_P, i-j]$
%      }
%    }
%  }
%}
%\Return{$A_P[r, k]$}
%\caption{\algo{MPA}: Message Passing Algorithm}
%\label{algo:mpa}
%\end{algorithm}
%
%
%% Message-Passing Algorithm
%\begin{algorithm}[h!]\label{alg}
%\SetAlgoNoLine
%\KwIn{$G = (V, E), T = (V_T, E_T), \sigma(\cdot), k$} % input
%\KwOut{$S \subset V$ such that $|S| = k$ %and $S$ maximizes $\sigma(\cdot)$ over the subsets of nodes associated with the nodes of $\mathcal{D}$
%} % output
%For a node $v_T \in V_T$, let $v_R, v_L,$ and $v_P$ be the left child, right child and parent of $v_T$, resp.
%Let $A_P[ \cdot , \cdot ] = V_T \times [k] \to 2^V$, such that $A_P[v_T,j]$ stores a
%choice of $j$ seeds in $T(v_T)$.  \\
%Let $A_L[ \cdot , \cdot ] = V_T \times [k] \to 2^V$, such that $A_L[v_T,j]$ stores a
%choice of $j$ seeds in $V \setminus T(v_L)$.  \\
%Let $A_R[ \cdot , \cdot ] = V_T \times [k] \to 2^V$, such that $A_R[v_T,j]$ stores a
%choice of $j$ seeds in $V \setminus T(v_R)$.  \\
%Let $r \in V_T$ be the root of $T$ and $h$ be its height.\\
%Run \algo{DPIM} on the input parameters, except return $A$ instead of the seed
%set. \\
%$A_P := A$ \\
%\While{$\sigma(A_P[r, k])$ is increasing } {
%  \For{each height $i = h - 1, h - 2, \ldots, 1, 2, \ldots h - 1$} {
%    \For{each node $v_T \in V_T$ with height $i$} {
%      \eIf{$v_T$ is the left child of $v_P$}{
%        $B := A_L$
%      }{
%        $B := A_R$
%      }
%      \For{each $i = 0, 1, \ldots, \min\{|T(v_T)|, k\}$}{
%        $j = \argmax\limits_{ j \in \{0, 1,\ldots, i\}} \sigma(A_P[ v_L,j] \cup
%        A_P[ v_R, i-j] \cup B[v_P, k - i])$\\
%        $A_P[v_T, i] = A_P[v_L, j] \cup A_P[v_R, i-j]$
%      }
%      \For{each $i = 0, 1, \ldots, \min\{|T(v_T)|, k\}$}{
%        $j = \argmax\limits_{ j \in \{0, 1,\ldots, i\}} \sigma(B[ v_P,j] \cup
%        A_P[ v_R, i-j] \cup A_P[v_L, k - i])$\\
%        $A_L[v_T, i] = B[v_P, j] \cup A_P[v_R, i-j]$
%      }
%      \For{each $i = 0, 1, \ldots, \min\{|T(v_T)|, k\}$}{
%        $j = \argmax\limits_{ j \in \{0, 1,\ldots, i\}} \sigma(A_P[ v_L,j] \cup
%        B[ v_P, i-j] \cup A_P[v_R, k - i])$\\
%        $A_R[v_T, i] = A_P[v_L, j] \cup B[v_P, i-j]$
%      }
%    }
%  }
%}
%\Return{$A_P[r, k]$}
%\caption{\algo{MPA}: Message Passing Algorithm}
%\label{algo:mpa}
%\end{algorithm}
%
\subsection{Message Passing Algorithm Evaluation}

We evaluate \algo{MPA} by comparing it's effectiveness against \algo{DPIM} for
all four cascades.  Due to the significant time complexity of \algo{MPA}, we were
only able to simulate \algo{MPA} on a small
network --- we sampled from the directed $(d, l, t)$-hierarchical network model
using parameters $(8, 15, 15)$.

As can be seen in Figure \ref{fig:mpa_eval}, the improvement that \algo{MPA} has
over \algo{DPIM} is marginal.  There are several possible explanations of these
results.  First, it is possible that the network we used in these simulations
does not have significant structure to support the cascade spreading faster via
inter-community synergies. Secondly, \algo{DPIM} could be inadvertently finding
the inter-community synergies. Or finally, for most networks, \algo{DPIM} is
good enough at finding the inter-community synergies for the specific cascade.
Whichever explanation is correct, our limited evaluation of this algorithm shows
that extending \algo{DPIM} to a message passing algorithm provides only marginal
improvements while taking much longer to execute.

  \begin{figure*}[hbtp]
    \begin{subfigure}{0.24\textwidth}
      \centering
      \input{fig/IndependentCascade.syn8d15c15a-txt}
      \caption{ICM}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
      \centering
      \input{fig/LinearThreshold.syn8d15c15a-txt}
      \caption{LTM}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
      \centering
      \input{fig/DeflatedIndependentCascade.syn8d15c15a-txt}
      \caption{DICM}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
      \centering
      \input{fig/GoyalContagion.syn8d15c15a-txt}
      \caption{SCM}
    \end{subfigure}

    \caption{\textbf{Evaluation of \algo{MPA}.} We evaluate the effectiveness of
    \algo{MPA}
    by comparing the results to \algo{DPIM}.  The network was a sample from the
    directed $(d,l,t)$- hierarchical network model using parameters (8,15,15).
    For each plot, the x-axis is $k$ and the y-axis is the expected total
    influence from the seed set chosen by each respective algorithm.}
    \label{fig:mpa_eval}
  \end{figure*}


==> test.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\begin{picture}(525,450)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(90.0,82.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(70,82){\makebox(0,0)[r]{$0$}}
\put(444.0,82.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(90.0,164.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(70,164){\makebox(0,0)[r]{$20$}}
\put(444.0,164.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(90.0,246.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(70,246){\makebox(0,0)[r]{$40$}}
\put(444.0,246.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(90.0,328.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(70,328){\makebox(0,0)[r]{$60$}}
\put(444.0,328.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(90.0,410.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(70,410){\makebox(0,0)[r]{$80$}}
\put(444.0,410.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(90.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(90,41){\makebox(0,0){$0$}}
\put(90.0,390.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(184.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(184,41){\makebox(0,0){$5$}}
\put(184.0,390.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(277.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(277,41){\makebox(0,0){$10$}}
\put(277.0,390.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(371.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(371,41){\makebox(0,0){$15$}}
\put(371.0,390.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(464.0,82.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(464,41){\makebox(0,0){$20$}}
\put(464.0,390.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(90.0,82.0){\rule[-0.200pt]{0.400pt}{79.015pt}}
\put(90.0,82.0){\rule[-0.200pt]{90.097pt}{0.400pt}}
\put(464.0,82.0){\rule[-0.200pt]{0.400pt}{79.015pt}}
\put(90.0,410.0){\rule[-0.200pt]{90.097pt}{0.400pt}}
\put(110,369){\makebox(0,0)[l]{DPIM}}
\put(250.0,369.0){\rule[-0.200pt]{24.090pt}{0.400pt}}
\put(90,82){\usebox{\plotpoint}}
\multiput(90.00,82.58)(0.680,0.494){25}{\rule{0.643pt}{0.119pt}}
\multiput(90.00,81.17)(17.666,14.000){2}{\rule{0.321pt}{0.400pt}}
\multiput(109.00,96.58)(0.528,0.495){31}{\rule{0.524pt}{0.119pt}}
\multiput(109.00,95.17)(16.913,17.000){2}{\rule{0.262pt}{0.400pt}}
\multiput(127.58,113.00)(0.495,0.605){35}{\rule{0.119pt}{0.584pt}}
\multiput(126.17,113.00)(19.000,21.787){2}{\rule{0.400pt}{0.292pt}}
\multiput(146.00,136.58)(0.964,0.491){17}{\rule{0.860pt}{0.118pt}}
\multiput(146.00,135.17)(17.215,10.000){2}{\rule{0.430pt}{0.400pt}}
\multiput(165.00,146.58)(0.634,0.494){27}{\rule{0.607pt}{0.119pt}}
\multiput(165.00,145.17)(17.741,15.000){2}{\rule{0.303pt}{0.400pt}}
\multiput(184.00,161.58)(0.755,0.492){21}{\rule{0.700pt}{0.119pt}}
\multiput(184.00,160.17)(16.547,12.000){2}{\rule{0.350pt}{0.400pt}}
\multiput(202.58,173.00)(0.495,0.605){35}{\rule{0.119pt}{0.584pt}}
\multiput(201.17,173.00)(19.000,21.787){2}{\rule{0.400pt}{0.292pt}}
\multiput(221.00,196.59)(1.408,0.485){11}{\rule{1.186pt}{0.117pt}}
\multiput(221.00,195.17)(16.539,7.000){2}{\rule{0.593pt}{0.400pt}}
\multiput(240.58,203.00)(0.495,0.526){33}{\rule{0.119pt}{0.522pt}}
\multiput(239.17,203.00)(18.000,17.916){2}{\rule{0.400pt}{0.261pt}}
\multiput(258.00,222.58)(0.734,0.493){23}{\rule{0.685pt}{0.119pt}}
\multiput(258.00,221.17)(17.579,13.000){2}{\rule{0.342pt}{0.400pt}}
\multiput(277.00,235.60)(2.674,0.468){5}{\rule{2.000pt}{0.113pt}}
\multiput(277.00,234.17)(14.849,4.000){2}{\rule{1.000pt}{0.400pt}}
\multiput(296.58,239.00)(0.495,0.583){33}{\rule{0.119pt}{0.567pt}}
\multiput(295.17,239.00)(18.000,19.824){2}{\rule{0.400pt}{0.283pt}}
\multiput(314.00,260.58)(0.964,0.491){17}{\rule{0.860pt}{0.118pt}}
\multiput(314.00,259.17)(17.215,10.000){2}{\rule{0.430pt}{0.400pt}}
\multiput(333.00,270.58)(0.498,0.495){35}{\rule{0.500pt}{0.119pt}}
\multiput(333.00,269.17)(17.962,19.000){2}{\rule{0.250pt}{0.400pt}}
\multiput(352.00,289.58)(0.798,0.492){21}{\rule{0.733pt}{0.119pt}}
\multiput(352.00,288.17)(17.478,12.000){2}{\rule{0.367pt}{0.400pt}}
\put(371,299.17){\rule{3.700pt}{0.400pt}}
\multiput(371.00,300.17)(10.320,-2.000){2}{\rule{1.850pt}{0.400pt}}
\multiput(389.58,299.00)(0.495,0.766){35}{\rule{0.119pt}{0.711pt}}
\multiput(388.17,299.00)(19.000,27.525){2}{\rule{0.400pt}{0.355pt}}
\multiput(408.00,328.59)(1.408,0.485){11}{\rule{1.186pt}{0.117pt}}
\multiput(408.00,327.17)(16.539,7.000){2}{\rule{0.593pt}{0.400pt}}
\multiput(427.00,335.58)(0.826,0.492){19}{\rule{0.755pt}{0.118pt}}
\multiput(427.00,334.17)(16.434,11.000){2}{\rule{0.377pt}{0.400pt}}
\multiput(445.58,346.00)(0.495,0.578){35}{\rule{0.119pt}{0.563pt}}
\multiput(444.17,346.00)(19.000,20.831){2}{\rule{0.400pt}{0.282pt}}
\put(90,82){\makebox(0,0){$\ast$}}
\put(109,96){\makebox(0,0){$\ast$}}
\put(127,113){\makebox(0,0){$\ast$}}
\put(146,136){\makebox(0,0){$\ast$}}
\put(165,146){\makebox(0,0){$\ast$}}
\put(184,161){\makebox(0,0){$\ast$}}
\put(202,173){\makebox(0,0){$\ast$}}
\put(221,196){\makebox(0,0){$\ast$}}
\put(240,203){\makebox(0,0){$\ast$}}
\put(258,222){\makebox(0,0){$\ast$}}
\put(277,235){\makebox(0,0){$\ast$}}
\put(296,239){\makebox(0,0){$\ast$}}
\put(314,260){\makebox(0,0){$\ast$}}
\put(333,270){\makebox(0,0){$\ast$}}
\put(352,289){\makebox(0,0){$\ast$}}
\put(371,301){\makebox(0,0){$\ast$}}
\put(389,299){\makebox(0,0){$\ast$}}
\put(408,328){\makebox(0,0){$\ast$}}
\put(427,335){\makebox(0,0){$\ast$}}
\put(445,346){\makebox(0,0){$\ast$}}
\put(464,368){\makebox(0,0){$\ast$}}
\put(300,369){\makebox(0,0){$\ast$}}
\put(110,328){\makebox(0,0)[l]{Greedy}}
\put(250.0,328.0){\rule[-0.200pt]{24.090pt}{0.400pt}}
\put(90,82){\usebox{\plotpoint}}
\multiput(90.00,82.59)(1.220,0.488){13}{\rule{1.050pt}{0.117pt}}
\multiput(90.00,81.17)(16.821,8.000){2}{\rule{0.525pt}{0.400pt}}
\multiput(109.00,90.58)(0.695,0.493){23}{\rule{0.654pt}{0.119pt}}
\multiput(109.00,89.17)(16.643,13.000){2}{\rule{0.327pt}{0.400pt}}
\multiput(127.58,103.00)(0.495,0.525){35}{\rule{0.119pt}{0.521pt}}
\multiput(126.17,103.00)(19.000,18.919){2}{\rule{0.400pt}{0.261pt}}
\multiput(146.00,123.58)(0.798,0.492){21}{\rule{0.733pt}{0.119pt}}
\multiput(146.00,122.17)(17.478,12.000){2}{\rule{0.367pt}{0.400pt}}
\multiput(165.58,135.00)(0.495,0.551){35}{\rule{0.119pt}{0.542pt}}
\multiput(164.17,135.00)(19.000,19.875){2}{\rule{0.400pt}{0.271pt}}
\multiput(184.00,156.59)(1.154,0.488){13}{\rule{1.000pt}{0.117pt}}
\multiput(184.00,155.17)(15.924,8.000){2}{\rule{0.500pt}{0.400pt}}
\multiput(202.58,164.00)(0.495,0.551){35}{\rule{0.119pt}{0.542pt}}
\multiput(201.17,164.00)(19.000,19.875){2}{\rule{0.400pt}{0.271pt}}
\multiput(221.00,185.60)(2.674,0.468){5}{\rule{2.000pt}{0.113pt}}
\multiput(221.00,184.17)(14.849,4.000){2}{\rule{1.000pt}{0.400pt}}
\multiput(240.58,189.00)(0.495,0.554){33}{\rule{0.119pt}{0.544pt}}
\multiput(239.17,189.00)(18.000,18.870){2}{\rule{0.400pt}{0.272pt}}
\multiput(258.58,209.00)(0.495,0.874){35}{\rule{0.119pt}{0.795pt}}
\multiput(257.17,209.00)(19.000,31.350){2}{\rule{0.400pt}{0.397pt}}
\multiput(277.00,240.92)(0.798,-0.492){21}{\rule{0.733pt}{0.119pt}}
\multiput(277.00,241.17)(17.478,-12.000){2}{\rule{0.367pt}{0.400pt}}
\multiput(296.58,230.00)(0.495,0.554){33}{\rule{0.119pt}{0.544pt}}
\multiput(295.17,230.00)(18.000,18.870){2}{\rule{0.400pt}{0.272pt}}
\multiput(314.00,250.59)(1.220,0.488){13}{\rule{1.050pt}{0.117pt}}
\multiput(314.00,249.17)(16.821,8.000){2}{\rule{0.525pt}{0.400pt}}
\multiput(333.00,258.59)(1.077,0.489){15}{\rule{0.944pt}{0.118pt}}
\multiput(333.00,257.17)(17.040,9.000){2}{\rule{0.472pt}{0.400pt}}
\multiput(352.58,267.00)(0.495,0.525){35}{\rule{0.119pt}{0.521pt}}
\multiput(351.17,267.00)(19.000,18.919){2}{\rule{0.400pt}{0.261pt}}
\multiput(371.00,287.59)(1.154,0.488){13}{\rule{1.000pt}{0.117pt}}
\multiput(371.00,286.17)(15.924,8.000){2}{\rule{0.500pt}{0.400pt}}
\multiput(389.00,295.58)(0.734,0.493){23}{\rule{0.685pt}{0.119pt}}
\multiput(389.00,294.17)(17.579,13.000){2}{\rule{0.342pt}{0.400pt}}
\multiput(408.00,308.60)(2.674,0.468){5}{\rule{2.000pt}{0.113pt}}
\multiput(408.00,307.17)(14.849,4.000){2}{\rule{1.000pt}{0.400pt}}
\multiput(427.58,312.00)(0.495,0.668){33}{\rule{0.119pt}{0.633pt}}
\multiput(426.17,312.00)(18.000,22.685){2}{\rule{0.400pt}{0.317pt}}
\multiput(445.00,336.58)(0.734,0.493){23}{\rule{0.685pt}{0.119pt}}
\multiput(445.00,335.17)(17.579,13.000){2}{\rule{0.342pt}{0.400pt}}
\put(90,82){\makebox(0,0){$\circ$}}
\put(109,90){\makebox(0,0){$\circ$}}
\put(127,103){\makebox(0,0){$\circ$}}
\put(146,123){\makebox(0,0){$\circ$}}
\put(165,135){\makebox(0,0){$\circ$}}
\put(184,156){\makebox(0,0){$\circ$}}
\put(202,164){\makebox(0,0){$\circ$}}
\put(221,185){\makebox(0,0){$\circ$}}
\put(240,189){\makebox(0,0){$\circ$}}
\put(258,209){\makebox(0,0){$\circ$}}
\put(277,242){\makebox(0,0){$\circ$}}
\put(296,230){\makebox(0,0){$\circ$}}
\put(314,250){\makebox(0,0){$\circ$}}
\put(333,258){\makebox(0,0){$\circ$}}
\put(352,267){\makebox(0,0){$\circ$}}
\put(371,287){\makebox(0,0){$\circ$}}
\put(389,295){\makebox(0,0){$\circ$}}
\put(408,308){\makebox(0,0){$\circ$}}
\put(427,312){\makebox(0,0){$\circ$}}
\put(445,336){\makebox(0,0){$\circ$}}
\put(464,349){\makebox(0,0){$\circ$}}
\put(300,328){\makebox(0,0){$\circ$}}
\put(90.0,82.0){\rule[-0.200pt]{0.400pt}{79.015pt}}
\put(90.0,82.0){\rule[-0.200pt]{90.097pt}{0.400pt}}
\put(464.0,82.0){\rule[-0.200pt]{0.400pt}{79.015pt}}
\put(90.0,410.0){\rule[-0.200pt]{90.097pt}{0.400pt}}
\end{picture}


==> time.tex <==
\subsection{The Running Time of \algo{DPIM}}
The analysis of the running time for \algo{DPIM} is straightforward.
\begin{theorem}
  Given a graph $G=(V,E)$ with $|V|=n,|E|=m$, fixed positive integers $k,r$, and a hierarchical decomposition $\mathcal{D}=(T,G)$, \algo{DPIM} has time complexity $O(mnk^2r)$, where $r$ is the number of times that $\sigma(\cdot)$ simulates the cascade, re-sampling the thresholds on each repetition.
\end{theorem}

\begin{proof}
  Observe that, for each node in $T$, \algo{DPIM} makes $O(k^2)$ queries to
  $\sigma(\cdot)$.  The execution of a single query to $\sigma(\cdot)$ has time
  complexity $O(mr)$, since simulating the cascade requires at most simulating
  the contagion on each edge in $G$.  The number of
  nodes in $T$ is exactly $2n-1$. %Consider an arbitrary agglomerative
  %hierarchical clustering algorithm. Starting with the $n$ leaves, the algorithm
 % creates an internal node in the hierarchical decomposition by combinining two
 % of these leaves.  Then, $n-1$ groups remain to be combined and $1$
  %internal node for $T$ was created. We continue this process of reducing the number of
 % groups by combining the groups together, increasing the number of internal
  %nodes in $T$, until there is only one group left.  Notice that the number of
 % times we combine two groups together is $n-1$.  So, the total number of nodes
  %in $T$ is $2n-1$.
   Hence, the running time of \algo{DPIM} is $O(mnk^2r)$.
\end{proof}

%\gs{is this right??}
%In comparison, the time complexity of the greedy algorithm is $O(n^2mkr)$, which is slower than \algo{DPIM} by a factor of $\frac nk$. 
